Porosities and dimensions of measures satisfying the doubling condition

Summary of a talk at the conference The Chaotic Universe in Rome, Feb, 1999

==> fig1.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point       2     4.5 {\clap{$z$}}
\point       1.8      5.5 {\clap{$p\,r$}}
\point       4.7     4.5 {\clap{$x$}}
\point       6     6.4 {\clap{$r$}}
 }}


==> lacundiv.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point      0.5   9.5 {\clap{{\eightpoint{$\max(p(r))$}}}}
\point      9      0.5 {\clap{{\eightpoint{$r$}}}}
\point      9    9 {\rlap{{\eightpoint{$n=6$}}}}
\point      9    8.55 {\rlap{{\eightpoint{$n=5$}}}}
\point      9    8.1 {\rlap{{\eightpoint{$n=4$}}}}
\point      9    7.65 {\rlap{{\eightpoint{$n=3$}}}}
 }}


==> lacunnodiv.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point      0.5   9.5 {\clap{{\eightpoint{$\rho$}}}}
\point      9      0.5 {\clap{{\eightpoint{$r$}}}}
\point      9    9 {\rlap{{\eightpoint{$n=6$}}}}
\point      9    8.55 {\rlap{{\eightpoint{$n=5$}}}}
\point      9    8.1 {\rlap{{\eightpoint{$n=4$}}}}
\point      9    7.65 {\rlap{{\eightpoint{$n=3$}}}}
 }}

